LEAD: Latent Realignment for Human Motion Diffusion

Our goal is to generate realistic human motion from natural language. Modern methods often face a trade-off between model expressiveness and text-to-motion alignment. Some align text and motion latent spaces but sacrifice expressiveness; others rely on diffusion models producing impressive motions, but lacking semantic meaning in their latent space. This may compromise realism, diversity, and applicability. Here, we address this by combining latent diffusion with a realignment mechanism, producing a novel, semantically structured space that encodes the semantics of language. Leveraging this capability, we introduce the task of textual motion inversion to capture novel motion concepts from a few examples. For motion synthesis, we evaluate LEAD on HumanML3D and KIT-ML and show comparable performance to the state-of-the-art in terms of realism, diversity, and text-motion consistency. Our qualitative analysis and user study reveal that our synthesized motions are sharper, more human-like and comply better with the text compared to modern methods. For motion textual inversion, our method demonstrates improved capacity in capturing out-of-distribution characteristics in comparison to traditional VAEs.

==> README <==
Created by Torsten Moeller, April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016
modified by Cagatay Turkay and Soumya Dutta, September 2019
modified by Cody Dunne, January and March 2023

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used with an established LaTeX environment by calling pdfLaTeX or LaTex. For online collaborative editing or without a local LaTeX installation, one option is to use https://www.overleaf.com/. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Unix-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> tune/sec/suppmat.tex <==
\clearpage
\setcounter{page}{1}
\maketitlesupplementary
\renewcommand \thesection{\arabic{section}}
\renewcommand\thesubsection{\Alph{subsection}}


\paragraph{Video}
We provide animated qualitative results and comparisons to baselines in the \textbf{supplementary video}. We compare text-to-motion results of \modelname with those generated using  T2M~\cite{Guo:2022}, MDM~\cite{Tevet:2022} and our reference method, MLD~\cite{Chen:2023}. In addition, we demonstrate qualitative results for the task of motion textual inversion.

\paragraph{Inference Time}
We provide a comparison in terms of inference times between \modelname and MLD~\cite{Chen:2023}. Tab.~\ref{tab:inference_time} shows the average inference time per sample across the whole test set in seconds. We find that the performance benefits of \modelname come with marginally increased computational overhead compared to MLD~\cite{Chen:2023}.

\begin{table}[h!]
    \centering
    \begin{tabular}{c|c}
       MLD~\cite{Chen:2023}  & \modelname \\
       \toprule
        0.236s &  0.245s
    \end{tabular}
    \caption{Average inference time per sample across the test-set, in seconds.}
    \label{tab:inference_time}
\end{table}

\paragraph{Limitations}
As demonstrated quantitatively and reflected by the user study, compared to the baselines, motions generated with \modelname are more realistic. However, they still sometimes exhibit motion artifacts such as foot-sliding. Furthermore, for long and sequential textual descriptions \modelname may struggle to produce motions that faithfully comply to the motion description. Finally, even though \modelname can generate arbitrary-length motions due to its design, it remains bounded by the maximum motion length present in the dataset.


\subsection{Projector Architecture}
\label{sec:rationale}
The projector is realised as a transformer-based encoder/decoder. The encoder and decoder both consist of 9 layers with 4 heads and hidden size 1024. We use 0.1 dropout and the GeLu activation function~\cite{Hendrycks:2016:GELU}. We use sinusoidal positional encodings.


\subsection{User Study}
\label{sec:rationale}
For the user study, we select motions generated using \modelname and MLD, conditioned on textual descriptions from HumanML3D~\cite{Guo:2022}. Our selection is based on the criterion of how much the motion differs before and after the realignment. We enlisted 40 participants with various age, gender and knowledge background (see Fig.~\ref{fig:stats1}, \ref{fig:stats2}). Our results in terms of average motion realism and text-motion relevance can be seen in Fig.~\ref{fig:res1}, and clearly demonstrate a preference over our method.

\begin{figure}
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{tune/figures/user_study_stats1.pdf}
\end{subfigure}%
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{tune/figures/user_study_stats2.pdf}
\end{subfigure}%

\caption{Gender and Age demographics of user study.}
\label{fig:stats1} 
\includegraphics[width=1\linewidth]{tune/figures/user_study_stats3.pdf}
\caption{Familiarity of participants with computer animation.}
\label{fig:stats2}  
\end{figure}



\begin{figure}
\centering
\begin{subfigure}{.25\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{tune/figures/user_study_results1.pdf}
  \caption{A subfigure}
 \label{fig:res1}
\end{subfigure}%
\begin{subfigure}{.255\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{tune/figures/user_study_results2.pdf}
  \caption{A subfigure}
  \label{fig:res1}
\end{subfigure}
\caption{User study results. As we can see, motions generated with \modelname are consistently perceived as more realistic than those generated using our reference method, MLD~\cite{Chen:2023}. In addition, motions generated with \modelname demonstrate higher scores on text-motion relevance in comparison to MLD, suggesting that our motions are perceived as more relevant to the conditioning texts. }
\label{fig:res1}
\end{figure}

\subsection{Data and Motion Representation}
\label{sec:rationale}
For the task of motion textual inversion we perform all our quantitative comparisons on a randomly chosen subset of 100 motions from HumanML3D. This is due to the fact that we first need to optimize one placeholder token for each motion, which requires significant time. In addition, we pre-process motions from 100styles dataset~\cite{Mason:2018} and convert them to the HumanML3D representation using the official implementation code from~\cite{Guo:2022}.
For the HumanML3D, format each motion $\mathbf{x} \in \mathbb{R}^{N \times D}$ is expressed redundantly as $\mathbf{x} = \{\dot{r}_a, \dot{r}_x, \dot{r}_z, r_y,\mathbf{j}_p, \mathbf{j}_v, \mathbf{j}_r,\mathbf{c}_f \}$ that consists of:
\begin{itemize}
     \item  root angular velocity $\dot{r}_a \in \mathbb{R}$ along the Y-axis,
     \item  root linear velocity $\dot{r}_x, \dot{r}_z \in \mathbb{R}$ along the XZ-axis,
     \item root height $r_y \in \mathbb{R}$,
     \item local joint positions $\mathbf{j}_p \in \mathbb{R}^{3N_j}$,
     \item local joint velocities  $\mathbf{j}_v \in \mathbb{R}^{3N_j}$,
     \item local joint rotations  $\mathbf{j}_r \in \mathbb{R}^{6N_j}$ in the root space,
    \item binary foot contact labels $\mathbf{c}_f \in \mathbb{R}^{4}$ that are obtained by thresholding on the velocities of the heel and toe joints.
\end{itemize}
Here, $N_j$ denotes the number of joints ($N_J=22$ for the HumanML3D dataset and $N_j=21$ for KIT-ML). 


\subsection{Evaluation Metrics}
\label{sec:rationale}
Here we provide the formulas for the metrics used in our quantitative evaluation.
\textbf{Realism} is assessed using the Fréchet Inception Distance (\textbf{FID}), calculated as:
\begin{equation}
    \text{FID} = \mid \mid \mu_r - \mu_g \mid \mid^2 + Tr(\Sigma_r + \Sigma_g - 2(\Sigma_r\Sigma_g)^{\frac{1}{2}}),
\end{equation}
where $\mu_r,\Sigma_r$ and $\mu_g,\Sigma_g$ correspond to the mean and covariance matrix of the real and generated motions respectively. 

\textbf{Multi-modal distance} (MMdist) is calculated as:
\begin{equation}
    \text{MMdist} = \frac{1}{N} \sqrt{(\sum_{i=1}^{N} \|  v_i - t_i\|)}
\end{equation}
where $v_i$ are the features of the motions generated using texts $y_i$, and $t_i$ are the features of the corresponding texts, $y_i$.

For \textbf{R-precision}, following Guo~\etal~\cite{Guo:2022}, for each generate motion we select its ground-truth textual description along with 31 randomly selected mismatched descriptions. Then we calculate the Euclidean distances between the motion feature and the 32 text features and rank them based on the distance. We select the top-1, top-2 and top-3 and consider as successful retrieval when the corresponding real text falls into the top-k candidates. R-precision is computed as the average across all generated motions from the test set. 

The \textbf{diversity} is calculated between the feature space of two randomly sampled sets of generated motions. For a subset of size $p$ the diversity can be computed as:
\begin{equation}
    \text{DIV} = \frac{1}{p}\sum_{i=1}^p\mid\mid v_i - \hat{v}_i \mid\mid
\end{equation}
where $v_i$, and $\hat{v}_i$ are the features corresponding to the first and second subset of predictions respectively. Following previous work~\cite{Chen:2023}, we set $p=300$. 

To calculate \textbf{MModality} (multimodality) we sample $m$ textual descriptions. For each description we generate two subsets of motions of size d. Then MModality is computed as:
\begin{equation}
    \text{MModality} = \frac{1}{m \times d}\sum_{j=1}^m\sum_{i=1}^d\mid\mid v_{j,i} - \hat{v}_{j,i} \mid \mid
\end{equation}
where $v$ and $\hat{v}$ are the motion features of each subset. Following~\cite{Chen:2023} we set $m=100$ and $d=10$. 

\subsection{Motion Textual Inversion}
\paragraph{Template texts} When learning the pseudo-word of the new concept we use predefined template texts to guide the diffusion model. We define the template texts using examples from the HumanML3D dataset. Below we provide some examples of template texts: 
\begin{itemize}
    \item the sim $<$*$>$.
    \item the man/woman $<$*$>$.
    \item figure $<$*$>$.
    \item someone $<$*$>$.
    \item he/she $<$*$>$.
    \item  a robot $<$*$>$.
\end{itemize}


